Simulation of a Microfluidic Gradient Generator using Lattice Boltzmann Methods

Microfluidics provides a powerful and versatile technology to accurately control spatial and temporal conditions for cell culturing and can therefore be used to study cellular responses to gradients. Here we use Lattice Boltzmann methods (LBM) to solve both the Navier-Stokes equation (NSE) for the fluid and the coupled convection-diffusion equation (CDE) for the compounds that form the diffusion-based gradient. The design of a microfluidic chamber for diffusion-based gradients must avoid flow through the cell chamber. This can be achieved by alternately opening the source and the sink channels. The fast toggling of microfluidic valves requires switching between different boundary conditions. We demonstrate that the LBM is a powerful method for handling complex geometries, high Peclet number conditions, discontinuities in the boundary conditions, and multiphysics coupling.

==> MyCollection <==
@article{Ayodele2011,
author = {Ayodele, S. and Varnik, F. and Raabe, D.},
doi = {10.1103/PhysRevE.83.016702},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ayodele, Varnik, Raabe - 2011 - Lattice Boltzmann study of pattern formation in reaction-diffusion systems.pdf:pdf},
issn = {1539-3755},
journal = {Physical Review E},
month = jan,
number = {1},
pages = {1--14},
title = {{Lattice Boltzmann study of pattern formation in reaction-diffusion systems}},
url = {http://link.aps.org/doi/10.1103/PhysRevE.83.016702},
volume = {83},
year = {2011}
}
@article{BARTOLONI1993,
author = {Bartoloni, A. and Battista, C. and Cabasino, S. and Paolucci, P. S. and Pech, J. and Sarno, R. and Todesco, G. M. and Torelli, M. and TROSS, W. and VICINI, P. and BENZI, R. and CABIBBO, N. and MASSAIOLI, F. and TRIPICCIONE, R.},
doi = {10.1142/S012918319300077X},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/BARTOLONI et al. - 1993 - LBE SIMULATIONS OF RAYLEIGH-B\'{E}NARD CONVECTION ON THE APE100 PARALLEL PROCESSOR.pdf:pdf},
issn = {0129-1831},
journal = {International Journal of Modern Physics C},
month = oct,
number = {05},
pages = {993--1006},
title = {{LBE Simulations of Rayleigh-B\'{e}nard convection on the APE100 Parallel Processor}},
url = {http://www.worldscientific.com/doi/abs/10.1142/S012918319300077X},
volume = {04},
year = {1993}
}
@article{Blaak2000,
author = {Blaak, Ronald and Sloot, Peter},
doi = {10.1016/S0010-4655(00)00112-0},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Blaak, Sloot - 2000 - Lattice dependence of reaction-diffusion in lattice Boltzmann modeling.pdf:pdf},
issn = {00104655},
journal = {Computer Physics Communications},
keywords = {lattice symmetry,lattice-boltzmann method,pattern formation,reaction-diffusion},
month = jul,
number = {1-3},
pages = {256--266},
title = {{Lattice dependence of reaction-diffusion in lattice Boltzmann modeling}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0010465500001120},
volume = {129},
year = {2000}
}
@article{Chen1998,
author = {Chen, Shiyi and Doolen, Gary D},
doi = {10.1146/annurev.fluid.30.1.329},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Chen, Doolen - 1998 - Lattice Boltzmann Methods for Fluid Flows.pdf:pdf},
issn = {0066-4189},
journal = {Annual Review of Fluid Mechanics},
keywords = {fluid flow simulation,lattice boltzmann method,mesoscopic approach},
month = jan,
number = {1},
pages = {329--364},
title = {{Lattice Boltzmann Methods for Fluid Flows}},
url = {http://www.annualreviews.org/doi/abs/10.1146/annurev.fluid.30.1.329},
volume = {30},
year = {1998}
}
@article{Chopard2009,
author = {Chopard, B. and Falcone, J. L. and Latt, J.},
doi = {10.1140/epjst/e2009-01035-5},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Chopard, Falcone, Latt - 2009 - The lattice Boltzmann advection-diffusion model revisited.pdf:pdf},
issn = {1951-6355},
journal = {The European Physical Journal Special Topics},
month = may,
number = {1},
pages = {245--249},
title = {{The lattice Boltzmann advection-diffusion model revisited}},
url = {http://www.springerlink.com/index/10.1140/epjst/e2009-01035-5},
volume = {171},
year = {2009}
}
@article{Frank2013,
abstract = {An automated microfluidic cell culture platform that creates and maintains independently programmable diffusion-based gradients is reported. Temporal modulation of the source and sink flow patterns allow generation of extremely stable spatial gradients. We developed a system that integrates 30 parallel gradients in a single device, with 10 different chemical formulations and 3 replicates. Mammalian fibroblast and macrophage cells were screened for NF$\kappa$B pathway activity under gradients of TNF$\alpha$, PDGF, and LPS, and multiparameter measurements were performed to demonstrate the capability of the device in dynamic single-cell analysis.},
author = {Frank, Tino and Tay, Savaş},
doi = {10.1039/c3lc41076e},
file = {:home/tanakas/Documents/01\_LITERATURE/01\_tanakas\_papers/frankTay2013.pdf:pdf},
issn = {1473-0189},
journal = {Lab on a chip},
month = apr,
number = {7},
pages = {1273--81},
pmid = {23386049},
title = {{Flow-switching allows independently programmable, extremely stable, high-throughput diffusion-based gradients.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/23386049},
volume = {13},
year = {2013}
}
@article{Guo2002b,
author = {Guo, Zhaoli and Shi, Baochang and Zheng, Chuguang},
doi = {10.1002/fld.337},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guo, Shi, Zheng - 2002 - A coupled lattice BGK model for the Boussinesq equations.pdf:pdf},
issn = {0271-2091},
journal = {International Journal for Numerical Methods in Fluids},
keywords = {lattice bgk method,natural convection,porous plate problem},
month = jun,
number = {4},
pages = {325--342},
title = {{A coupled lattice BGK model for the Boussinesq equations}},
url = {http://doi.wiley.com/10.1002/fld.337},
volume = {39},
year = {2002}
}
@article{Guo2002a,
author = {Guo, Zhaoli and Zheng, Chuguang and Shi, B.C.},
doi = {10.1063/1.1471914},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guo, Zheng, Shi - 2002 - An extrapolation method for boundary conditions in lattice Boltzmann method.pdf:pdf},
issn = {10706631},
journal = {Physics of Fluids},
number = {6},
pages = {2007},
title = {{An extrapolation method for boundary conditions in lattice Boltzmann method}},
url = {http://link.aip.org/link/PHFLE6/v14/i6/p2007/s1\&Agg=doi},
volume = {14},
year = {2002}
}
@article{HEYWOOD1996,
author = {Heywood, J. G. and Rannacher, R. and Turek, S.},
doi = {10.1002/(SICI)1097-0363(19960315)22:5<325::AID-FLD307>3.0.CO;2-Y},
file = {:home/tanakas/Documents/01\_LITERATURE/01\_tanakas\_papers/HeywoodRannacherTurek1996.pdf:pdf},
issn = {0271-2091},
journal = {International Journal for Numerical Methods in Fluids},
keywords = {dficial boundq conditions,finite elwcnts,flux and pessure conditions,navicrstokes equations},
month = mar,
number = {5},
pages = {325--352},
title = {{Artificial Boundaries and Flux and Pressure Conditions for the Incompressible Navier-Stokes Equations}},
url = {http://doi.wiley.com/10.1002/\%28SICI\%291097-0363\%2819960315\%2922\%3A5\%3C325\%3A\%3AAID-FLD307\%3E3.0.CO\%3B2-Y},
volume = {22},
year = {1996}
}
@article{Hu2011,
author = {Hu, Yangxu and Zhang, Xianren and Wang, Wenchuan},
doi = {10.1021/ie201136r},
file = {:home/tanakas/Documents/01\_LITERATURE/01\_tanakas\_papers/HuZhangWang2011.pdf:pdf},
issn = {0888-5885},
journal = {Industrial \& Engineering Chemistry Research},
month = dec,
number = {24},
pages = {13932--13939},
title = {{Simulation of the Generation of Solution Gradients in Microfluidic Systems Using the Lattice Boltzmann Method}},
url = {http://pubs.acs.org/doi/abs/10.1021/ie201136r},
volume = {50},
year = {2011}
}
@article{Inamuro2002,
abstract = {A lattice kinetic scheme for incompressible viscous flows with heat transfer is developed based on the lattice Boltzmann method. In the new scheme, macroscopic variables are calculated without velocity distribution functions. Thus, the scheme can save computer memory because there is no need to store the velocity distribution functions. Governing equations for the macroscopic variables are obtained by applying the asymptotic theory. The continuity equation, the Navier-Stokes equations, and the convection-diffusion equation for fluid temperature are obtained with relative errors of O(epsilon2), where epsilon is a small parameter that is of the same order as a lattice spacing and is related to a relaxation parameter. In order to verify the accuracy of the scheme, natural convection flows in a square cavity are simulated, and the calculated results are in good agreement with available standard results.},
author = {Inamuro, Takaji},
doi = {10.1098/rsta.2001.0942},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Inamuro - 2002 - A lattice kinetic scheme for incompressible viscous flows with heat transfer.pdf:pdf},
issn = {1364-503X},
journal = {Philosophical transactions. Series A, Mathematical, physical, and engineering sciences},
keywords = {Chemical,Colloids,Colloids: chemistry,Computer Simulation,Crystallization,Crystallization: methods,Diffusion,Energy Transfer,Gases,Gases: chemistry,Hot Temperature,Kinetics,Models,Particle Size,Pressure,Quantum Theory,Rheology,Rheology: methods,Statistical},
month = mar,
number = {1792},
pages = {477--84},
pmid = {16210191},
title = {{A lattice kinetic scheme for incompressible viscous flows with heat transfer.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/16210191},
volume = {360},
year = {2002}
}
@article{Li2001,
author = {Li, Qing and Zheng, C.G. and Wang, N.C. and Shi, B.C.},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Li et al. - 2001 - LBGK simulations of Turing patterns in CIMA model.pdf:pdf},
journal = {Journal of scientific computing},
keywords = {cima model,lattice boltzmann method,patterns,reaction-diffusion equation,turing},
number = {2},
pages = {121--134},
publisher = {Springer},
title = {{LBGK simulations of Turing patterns in CIMA model}},
url = {http://www.springerlink.com/index/wk8t2587642v7221.pdf},
volume = {16},
year = {2001}
}
@article{PonceDawson1993,
author = {{Ponce Dawson}, S. and Chen, S and Doolen, Gary D},
doi = {10.1063/1.464316},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ponce Dawson, Chen, Doolen - 1993 - Lattice Boltzmann computations for reaction-diffusion equations.pdf:pdf},
issn = {00219606},
journal = {The Journal of Chemical Physics},
keywords = {BOLTZMANN EQUATION,CALCULATION METHODS,CHEMICAL REACTIONS,CONVECTION,DIFFUSION,FLUID FLOW,PATTERN RECOGNITION,SIMULATION,VELOCITY},
number = {2},
pages = {1514},
title = {{Lattice Boltzmann computations for reaction-diffusion equations}},
url = {http://link.aip.org/link/?JCPSA6/98/1514/1 http://link.aip.org/link/JCPSA6/v98/i2/p1514/s1\&Agg=doi},
volume = {98},
year = {1993}
}
@article{Suga2006,
author = {Suga, Shinsuke},
doi = {10.1142/S0129183106010030},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Suga - 2006 - Numerical schemes obtained from lattice boltzmann equations for advection diffusion equations.pdf:pdf},
journal = {International Journal of Modern Physics C},
keywords = {accuracy of the scheme,advection-diffusion,lattice boltzmann equation,scheme,stability of the numerical},
number = {11},
pages = {1563--1577},
title = {{Numerical schemes obtained from lattice boltzmann equations for advection diffusion equations}},
volume = {17},
year = {2006}
}
@article{Wolf-Gladrow1995,
author = {Wolf-Gladrow, Dieter},
doi = {10.1007/BF02181215},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wolf-Gladrow - 1995 - A lattice Boltzmann equation for diffusion.pdf:pdf},
issn = {0022-4715},
journal = {Journal of Statistical Physics},
keywords = {1,10 years h a,a l m e,d d e v,diffusion,e l o p,e r i c,explicit schemes,finite differences,i n t r,lattice boltzmann equation,m e n t,numerical stability,o d u c,o f n e,r a p i,s,t h e last,t h o d,t i o n,underrelaxation,v e seen a,w n u m},
month = jun,
number = {5-6},
pages = {1023--1032},
title = {{A lattice Boltzmann equation for diffusion}},
url = {http://www.springerlink.com/index/10.1007/BF02181215},
volume = {79},
year = {1995}
}
@article{Zhang2006a,
author = {Zhang, Junfeng and Kwok, Daniel},
doi = {10.1103/PhysRevE.73.047702},
file = {:home/tanakas/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zhang, Kwok - 2006 - Pressure boundary condition of the lattice Boltzmann method for fully developed periodic flows.pdf:pdf},
issn = {1539-3755},
journal = {Physical Review E},
month = apr,
number = {4},
pages = {4--7},
title = {{Pressure boundary condition of the lattice Boltzmann method for fully developed periodic flows}},
url = {http://link.aps.org/doi/10.1103/PhysRevE.73.047702},
volume = {73},
year = {2006}
}
@article{Dertinger2001,
author = {Dertinger, Stephan K. W. and Chiu, Daniel T. and Jeon, Noo Li and Whitesides, George M.},
doi = {10.1021/ac001132d},
file = {:home/tanakas/Documents/01\_LITERATURE/01\_tanakas\_papers/DertingerChiuJeonWhitesides2001.pdf:pdf},
issn = {0003-2700},
journal = {Analytical Chemistry},
month = mar,
number = {6},
pages = {1240--1246},
title = {{Generation of Gradients Having Complex Shapes Using Microfluidic Networks}},
url = {http://pubs.acs.org/doi/abs/10.1021/ac001132d},
volume = {73},
year = {2001}
}


